Friendly Sharpness-Aware Minimization

Sharpness-Aware Minimization (SAM) has been instrumental in improving deep neural network training by minimizing both training loss and loss sharpness. Despite the practical success, the mechanisms behind SAM's generalization enhancements remain elusive, limiting its progress in deep learning optimization. In this work, we investigate SAM's core components for generalization improvement and introduce "Friendly-SAM" (F-SAM) to further enhance SAM's generalization. Our investigation reveals the key role of batch-specific stochastic gradient noise within the adversarial perturbation, i.e., the current minibatch gradient, which significantly influences SAM's generalization performance. By decomposing the adversarial perturbation in SAM into full gradient and stochastic gradient noise components, we discover that relying solely on the full gradient component degrades generalization while excluding it leads to improved performance. The possible reason lies in the full gradient component's increase in sharpness loss for the entire dataset, creating inconsistencies with the subsequent sharpness minimization step solely on the current minibatch data. Inspired by these insights, F-SAM aims to mitigate the negative effects of the full gradient component. It removes the full gradient estimated by an exponentially moving average (EMA) of historical stochastic gradients, and then leverages stochastic gradient noise for improved generalization. Moreover, we provide theoretical validation for the EMA approximation and prove the convergence of F-SAM on non-convex problems. Extensive experiments demonstrate the superior generalization performance and robustness of F-SAM over vanilla SAM. Code is available at https://github.com/nblt/F-SAM.

==> sec/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.50\linewidth]{figure/illustration2.png}
	\includegraphics[width=0.49\linewidth]{figure/intro-compare.pdf}
	\caption{Investigation on SAM's adversarial  perturbation direction. We decompose the minibatch gradient $\nabla_\mathcal{B} L(\boldsymbol{w})$ into two  components: the full gradient component and the remaining stochastic gradient noise.  Solely using the full gradient component leads to a dramatic generalization degradation, while only using the noise component enhances the generalization.}
% 	\caption{Illustration of F-SAM's accent direction for weight perturbation. Accenting towards the full gradient direction $\nabla L(\boldsymbol{w})$ contributes minimally to generalization and can potentially have a detrimental effect. We thus propose to eliminate the full gradient component, resulting our F-SAM perturbation. 
% This modified perturbation is less aggressive in terms of increasing loss compared to SAM's and significantly enhances the generalization. }
	\label{fig:illustration}
\end{figure} 
 

Deep neural networks (DNNs) have achieved remarkable performance in various vision and language processing tasks \cite{devlin2018bert, brown2020language, liu2021swin}. A critical factor contributing to their success is the choice of optimization algorithms \cite{robbins1951stochastic,kingma2014adam,loshchilov2017decoupled,zhuang2020adabelief,xie2022adan}, designed to efficiently optimize DNN model parameters. To achieve better performance, it is often desirable for an optimizer to converge to flat minima, characterized by uniformly low loss values, as opposed to sharp minima with abrupt loss changes, as the former typically results in better generalization \cite{hochreiter1997flat,dinh2017sharp, li2018visualizing,zhou2020towards}. However, the complex landscape of over-parameterized DNNs, featuring numerous sharp and flat minima, presents practical challenges for optimizers in real applications.


To address this challenge, Sharpness-Aware Minimization (SAM) \cite{foret2020sharpness} is proposed to simultaneously minimize the training loss  and the loss sharpness, enabling it to identify flat minima associated with improved generalization performance.  For each training iteration, given the minibatch training loss   $L_{\mathcal{B}}(\boldsymbol{w})$ parameterized by  $\boldsymbol{w}$, SAM achieves this by adversarially computing a weight perturbation  $\boldsymbol{\epsilon}_s$ to maximize  the   training loss  $L_{\mathcal{B}}(\boldsymbol{w}+\boldsymbol{\epsilon}_s)$. It then minimizes the loss of this perturbed objective via one updating step of a base optimizer, such as SGD~\citep{robbins1951stochastic}. In practice, to efficiently compute  $\boldsymbol{\epsilon}_s$,  SAM takes a linear approximation of the loss objective, and employs the minibatch gradient  $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ as the accent direction for searching $\boldsymbol{\epsilon}_s = \rho\cdot \norm(\nabla L_{\mathcal{B}}(\boldsymbol{w}))$, where $\norm(\boldsymbol{x})= \boldsymbol{x}/ \|\boldsymbol{x}\|_2$ and $\rho>0$ is a radius. This approach enables SAM to seek models situated in neighborhoods characterized by consistently low loss values, resulting in better generalization when used in conjunction with base optimizers such as SGD and Adam~\cite{kingma2014adam}. 


{Despite SAM's practical success, the underlying mechanism responsible for its empirical generalization improvements remains limited} \cite{andriushchenko2022towards,chen2023does},  though heavily desired.  This open challenge hinders developing new and more advanced deep learning optimization algorithms  in a principle way.  
To address this issue, we undertake a comprehensive exploration of SAM's core components contributing to its generalization improvement. Subsequently, we introduce a new variant of SAM, which offers a simple  yet  effective approach to further enhance the generalization  performance  in conjunction with popular base optimizers.
 
 

First, our investigations reveal that the stochastic gradient noise present in the minibatch gradient $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ plays a crucial role in SAM's generalization performance. Specifically,  as shown in Fig.~\ref{fig:illustration}, we decompose the perturbation direction $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ into two orthogonal components: the full gradient component $\mathrm{Proj}_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$, representing the projection of $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ onto the full gradient direction, and the stochastic gradient noise component $\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$, denoting the residual projection. Surprisingly, we  empirically find that  as shown in Fig.~\ref{fig:illustration},  using only the full gradient component for perturbation significantly degrades SAM's generalization, while excluding the full gradient component leads to improved performance. This observation suggests that the effectiveness of SAM primarily arises from the presence of the stochastic gradient noise component within the minibatch gradient $\nabla L_{\mathcal{B}}(\boldsymbol{w})$. The reason behind this phenomenon may be that the full gradient component in the perturbation increases the sharpness loss of the entire dataset, leading to inconsistencies with the subsequent sharpness minimization step which only uses the current minibatch data to minimize  training loss value and its sharpness.   See more discussion in Sec.~\ref{sec:investigation}. 

%To begin with,  our investigations reveal
%that the stochastic gradient noise present in the minibatch gradient $\nabla L_{\mathcal{B}}(\boldsymbol{w})$   plays a crucial role in the generalization performance of SAM.
%Specifically, as illustrated in Fig.~\ref{fig:illustration}, we decompose the perturbation direction  $\nabla L_{\mathcal{B}}(\boldsymbol{w})$   into two orthogonal components:  
%the full gradient component
%$\mathrm{Proj}_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$ that is the projection of  $\nabla L_{\mathcal{B}}(\boldsymbol{w})$  onto the full gradient direction, 
%and  
%the stochastic gradient noise component 
%$\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$, 
%representing the residual projection.
%Surprisingly, we empirically observe that as shown in Fig.~\ref{fig:illustration}, 1) solely using the full gradient component as the perturbation by setting   $\boldsymbol{\epsilon}_s =\rho \cdot \norm(\nabla L(\boldsymbol{w}))$ during each training iteration significantly degrades the generalization of SAM; 2) excluding the full gradient component by setting perturbation $\boldsymbol{\epsilon}_s = \rho \cdot \norm\big(\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})\big)$ improves the generalization performance.
%This intriguing observation indicates that the effectiveness of SAM primarily arises from the presence of stochastic gradient noise component within the minibatch gradient $\nabla L_{\mathcal{B}}(\boldsymbol{w})$. 
%The possible reason  behind this phenomenon is that  the full gradient component in the perturbation increases the sharpness loss of the entire dataset, while the subsequent minimization step  only uses the current minibatch data to minimize the sharpness. This inconsistency could    limit  the effective sharpness optimization.  See more discussion in Sec.~\ref{sec:investigation}.  

%Next, building on this insight, we introduce a straightforward yet highly effective modification to SAM, which we refer to as ``Friendly-SAM'' or F-SAM. The primary concept behind F-SAM is to mitigate the undesirable effects introduced by the full gradient component 
%within the minibatch gradient, 
%and  harness the beneficial role of stochastic gradient noise 
%to further enhance SAM's generalization performance. Intuitively, $\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$ serves as an ascent direction that maximizes the loss solely for the current minibatch data while minimizing its impact on other data points as much as possible. Therefore, the adversarial perturbation generated by F-SAM is more ``friendly'' to other data points compared with the original perturbation in SAM. 
%Such friendliness enables F-SAM being less sensitive to the choice of perturbation radius as discussed in \cref{sec:ablation}. For practical efficiency, F-SAM  approximates the computationally expensive full gradient through an exponentially moving average (EMA) of the historical stochastic gradients, and then computes the stochastic gradient noise as the perturbation direction. Moreover, we  theoretically shows  the validation of the EMA approximation to the full gradient approximation , and also proves the convergence of F-SAM  on the nonconvex problems. 

Next, building on this insight, we introduce a straightforward yet highly effective modification to SAM, referred to as ``Friendly-SAM" or F-SAM. F-SAM mitigates the undesirable effects of the full gradient component within the minibatch gradient and leverages the beneficial role of stochastic gradient noise to further enhance SAM's generalization performance.  Since removing full gradient component in the perturbation step can relieve the adversarial perturbation impact on other data points except for current minibatch data, the adversarial perturbation in F-SAM is more ``friendly'' to other data points compared with vanilla SAM, which helps the adversarial perturbation and the following minimization perform on the same minibatch data and improves sharpness minimization consistency.  Moreover, such friendliness enables F-SAM to be less sensitive to the choice of perturbation radius as discussed in \cref{sec:ablation}.  For efficiency,  F-SAM approximates the computationally expensive full gradient through an exponentially moving average (EMA) of the historical stochastic gradients and computes the stochastic gradient noise as the perturbation direction.  
Moreover, we also provide theoretical validation of the EMA approximation to the full gradient and prove the convergence of F-SAM on non-convex problems.  Our main contribution can be summarized as follows:
\begin{itemize}
	\item We take an in-depth investigation into the key component in SAM's adversarial perturbation and identify that the stochastic gradient noise plays the most significant role. 
	\item We propose a novel variant of SAM called F-SAM by eliminating the undesired full gradient component and harnesses the beneficial stochastic gradient noise for adversarial perturbation to enhance generalization. % Our modification can be readily applied to SAM's adaptive variants.
	\item Extensive experimental results demonstrates  that F-SAM improves SAM's generalization, aids in training, and exhibits better robustness across different perturbation radii.
\end{itemize}


% Deep neural networks (DNNs) have achieved remarkable performance in numerous vision and language tasks \cite{devlin2018bert, brown2020language, liu2021swin}.
% A crucial factor contributing to the tremendous success of DNNs lies in the optimization algorithms employed \cite{kingma2014adam,loshchilov2017decoupled,zhuang2020adabelief,xie2022adan}, 
% which aim to efficiently navigate the vast hypothesis space in search of satisfactory solutions. 
% Various optimizers have been designed to address different aspects of optimization properties.
% Notably, a recent innovation known as sharpness-aware minimization (SAM) \cite{foret2020sharpness} has been proposed, which demonstrates state-of-the-art generalization performance across various domains.

% SAM improves the generalization by formulating the optimization target as a min-max problem, aiming to minimize the sharpness measure of the loss landscape defined by a neighborhood maximization. Denote by  $L(\boldsymbol{w})$ the loss objective to be minimized (e.g., the cross-entropy loss for classification) with $\boldsymbol{w}$ being the model parameters. SAM first adversarially computes a weight perturbation $\boldsymbol{\epsilon}_s$ that maximizes $L(\boldsymbol{w}+\boldsymbol{\epsilon}_s)$, and subsequently minimizes the loss of the perturbed objective. However, due to the high complexity of this min-max optimization problem, SAM practically uses a linear approximation of $L(\boldsymbol{w})$ and determines the worst-case direction of the weight perturbation 
% through the gradient, i.e., $\nabla L(\boldsymbol{w})$ (refer to Section \ref{sec:preliminary} for details).

% Despite the empirical success of SAM, the underlying  mechanism that enables such significant improvements in generalization is yet not well understood. 
% In this paper, we aim to gain a deeper understanding of the key components that contribute to SAM's effective generalization.
% % to delve into a deeper understanding of the key components that contributes the SAM's effective generalization. 
% By examining the decomposition of the batch gradient $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ into two orthogonal components, i.e., the projection onto the full gradient direction and the residual projection, we observe that the full gradient component contributes little to the generalization of SAM.
% In fact, strengthening it can even have a detrimental effect on generalization. 
% This finding aligns with the intriguing phenomenon of $m$-sharpness, which is defined as the search for an adversarial perturbation that maximizes the sum of losses over batches of $m$ training points, as discussed in the previous literature \cite{foret2020sharpness, andriushchenko2022towards}. This phenomenon emphasizes the importance of using a low value for $m$ to effectively improve generalization \cite{foret2020sharpness, andriushchenko2022towards, behdin2022improved}, which implicitly reduces the influence of the full gradient component in the subbatch gradient.


\begin{figure*}[!t]
	\centering
	\begin{subfigure}{0.335\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{figure/sam-fb-new.pdf}
		\caption{}
		\label{fig:sam-fb}
	\end{subfigure}
	\hspace{0.02in}
	\begin{subfigure}{0.345\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{figure/sam-db-new.pdf}
		\caption{}  
		\label{fig:sam-db}
	\end{subfigure}
	\hspace{0.02in}
	\begin{subfigure}{0.26\linewidth}
		\centering
		\hspace{0.02in}
		\includegraphics[width=1\linewidth]{figure/strength.pdf}
		\caption{}  
		\label{fig:sam-strength}
	\end{subfigure}
	\caption{Performance comparison of different versions of SAM with SGD/AdamW as its base optimizer.  In (a),  SAM-full denotes the version of SAM using the full gradient component as the perturbation. In (b), SAM-db represents the SAM using different random-selected data batch for perturbation and its following minimization step.  (c) compares  SAM using different minibatch size to compute the perturbation but always fixing minibatch size of 128 for the following minimization step.} 
	\label{fig:investigation}
\end{figure*}

% This finding also coincides with the intriguing $m$-sharpness phenomenon \cite{foret2020sharpness,andriushchenko2022towards}, which is defined as searching for an adversarial perturbation $\boldsymbol{\epsilon}_s$ that maximizes the sum of losses over batches of $m$ training points. The m-sharpness phenomenon emphasizes the importance of using a low $m$ for effectively improve generalization \cite{foret2020sharpness, andriushchenko2022towards,behdin2022improved}. 


% One of the intriguing aspects is known as $m$-sharpness \cite{foret2020sharpness}, which is defined as searching for an adversarial perturbation $\boldsymbol{\epsilon}_s$ that maximizes the sum of losses over batches of $m$ training points. 
% Numerous studies have emphasized the importance of using a low $m$ for effectively improve generalization \cite{foret2020sharpness, andriushchenko2022towards,behdin2022improved}. 
% In fact, it has been shown that as $m$ increases to the total number of training data $n$, the effect of generalization improvement diminishes compared with empirical risk minimization (ERM) without weight perturbation \cite{andriushchenko2022towards}.
% This interesting phenomenon suggests that the practical success of SAM may not solely rely on minimizing the sharpness of the global loss objective.

%  may do not necessarily rely on minimizing the sharpness of the ``global'' loss objective. Instead, it indicates that more ``local'' training behavior related to each training step needs to be considered.

% In this work, we delve deeper into this phenomenon by examining the decomposition of the batch gradient $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ into two orthogonal components: the projection onto the full gradient direction and the residual projection (as illustrated in Figure X). 
% The former component is responsible for increasing the loss over the full training data, while both components combined  contribute to increasing the loss over the current batch data. 
% We then investigate  the role of these components in enhancing  generalization.
% Being aware that the full batch version of SAM does not yield generalization improvement compared to ERM, we hypothesis that only accent towards the remaining part of the projection contributes the practical generalization improvement of SAM, while accent towards to full gradient direction  $\nabla L(\boldsymbol{w})$ does not.

% % experimental justification
% We further support the hypothesis by introducing a modified version of SAM called SAM-db [XX], where we utilize two different data batches for SAM's accent and descent steps, respectively. The only distinction between SAM and SAM-db is that in SAM, the gradient noise in both steps is consistent while in SAM-db, they are associated with different data batches. In Figure X,  we observe that SAM-db still does not bring any generalization improvement compared to ERM.
% If optimizing the global sharpness with $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ truly contributes to generalization, we should still observe at least slight generalization improvement over ERM, as the global sharpness is still optimized.

% convergence benefits

% The presence of such full gradient accent component can hinder the training process by increasing the loss over the entire datasets and even have a negative impact on generalization, as detailed in Section \ref{sec:investigation}. Therefore, we propose to eliminate the component that contributes the increase in the loss over the entire dataset during SAM's accent step.
% However, computing the full gradient for each iteration during the training is infeasible. Instead, we estimate the full gradient practically by employing an exponentially moving average (EMA) with historical gradients. 
% Nevertheless, this approximation unavoidably introduces noise into the estimation of the full gradient, thereby reducing the reliability of the gradient projection operation. To tackle this challenge, we further propose a simple approach via gradient subtraction to appropriately bypass the projection operation (as illustrated in Figure \ref{fig:illustration}), which is expected to be more effective in eliminate the full gradient component under noise setting.

% and effectively eliminate the full gradient component in the accent direction. 



% By removing the full gradient accent component, our adjusted accent direction is expected to be less aggressive towards the global loss objective. Therefore, we name our approach Friendly-SAM (F-SAM). To differentiate it from SAM, we further formulate our optimization target as a bi-level optimization problem [X] and interpret the accent direction of F-SAM from a brand new perspective --- 
% in contrast to the original SAM, which searches for an ascent direction that maximizes the loss of the current batch data, we aim to find a direction that increases the loss of the current batch data while minimizing the impact on other data points as much as possible. 
% Our modification can also be readily applied to SAM's variants that with improved geometric measures.
% We conduct extensive experiments over various tasks to demonstrate that F-SAM not only improves the convergence compared with SAM but also brings consistently generalization improvement.
% % conclusion

% In summary, we make the following contributions:


% \section{Related Work}

% \section{Preliminaries}
% \label{sec:preliminary}
% Let $f(\boldsymbol{x};\boldsymbol{w})$ denote a neural network function with trainable parameters $\boldsymbol{w} \in \mathbb{R}^d$, where $d$ represents the number of parameters. The loss function for a pair of data points $(\boldsymbol{x}_i,\boldsymbol{y}_i)$ is denoted as $L(f(\boldsymbol{x}_i;\boldsymbol{w}), \boldsymbol{y}_i)$ (short for $L_i(\boldsymbol{w})$). We are given a dataset $\mathcal{S}={ (\boldsymbol{x}_i,\boldsymbol{y}_i) }_{i=1}^n$ drawn from a data distribution $\mathcal{D}$ under the assumption of independent and identically distributed (i.i.d.) conditions. The empirical loss is defined as $L(\boldsymbol{w})= \frac{1}{n}\sum_{i=1}^nL_i(\boldsymbol{w})$, which represents the average loss over the entire dataset.

% Sharpness-Aware Minimization (SAM) is an optimization technique introduced in the paper by Foret et al. \cite{foret2020sharpness}. SAM aims to minimize the worst-case loss within a defined neighborhood, represented by a norm ball, in order to bias the training process towards flat minima. The objective function of SAM is given by:
% \begin{equation}
	%     L^{\rm SAM}(\boldsymbol{w})= \max_{\| \boldsymbol{\epsilon} \|_2 \le \rho} L(\boldsymbol{w}+\boldsymbol{\epsilon}),
	%     \label{equ:sam}
	% \end{equation}
% where $\rho$ denotes the radius that determines the size of the neighborhood. In this formulation, SAM seeks to minimize the maximum loss over the neighborhood surrounding the current weight configuration, $\boldsymbol{w}$. By doing so, SAM encourages the optimization process to converge to flat minima.

% In order to optimize $L^{\rm SAM}$, the worst-case perturbations $\boldsymbol{\epsilon}$ need to be determined for the maximization problem. Foret et al. \cite{foret2020sharpness} propose a practical approximation of (\ref{equ:sam}) using a first-order expansion. The approximate expression for $\boldsymbol{\epsilon}_s$ is given by:
% \begin{equation}
	%     \boldsymbol{\epsilon}^*\approx \mathop{ \arg \max}\limits_{\| \boldsymbol{\epsilon} \|_2\le \rho} \boldsymbol{\epsilon}_s ^{\top} \nabla_{\boldsymbol{w}} L(\boldsymbol{w})= \rho \frac{\nabla_ {\boldsymbol{w}} L(\boldsymbol{w})}{\| \nabla_{\boldsymbol{w}} L(\boldsymbol{w}) \|_2}.
	%     \label{equ:sam-first-order}
	% \end{equation}
% Subsequently, the gradient at the perturbed weight $\boldsymbol{w}+\boldsymbol{\epsilon}^*_s$ is computed to update the model:
% \begin{equation}
	% \nabla L^{\rm SAM} (\boldsymbol{w}) \approx
	% \nabla L (\boldsymbol{w}) |_{\boldsymbol{w}+\boldsymbol{\epsilon}_s^*}.
	% \end{equation}
\section{Related Work}

\textbf{Sharp Minima and Generalization.}
The connection between the flatness of local minima and generalization has received a rich body of studies \cite{hochreiter1997flat, chaudhari2017entropy, keskar2017large,dinh2017sharp, izmailov2018averaging, li2018visualizing}.
Recently, many works try to improve the model generalization by seeking flat minima \cite{chaudhari2017entropy, wen2018smoothout, tsuzuku2020normalized, foret2020sharpness, zheng2021regularizing, bisla2022low, li2022efficient}. For example, Chaudhari et al. \cite{chaudhari2017entropy} propose Entropy-SGD that actively searches for flat regions by minimizing local entropy.
Wen et al. \cite{wen2018smoothout} propose SmoothOut framework to smooth out the sharp minima and obtain generalization improvements.
Notably, sharpness-aware minimization (SAM) \cite{foret2020sharpness} provides a generic training scheme for seeking flat minima by formulating the optimization as a min-max problem and encourage parameters sitting in neighborhoods with uniformly low loss, achieving state-of-the-art generalization improvements across various tasks. 
% The original SAM defines the neighborhood using $\ell_2$-norm, which does not precisely conform with the natural geometry of loss function.
Later, a line of works improves SAM from the perspective of the neighborhood's geometric measure \cite{kwon2021asam, kim2022fisher}, surrogate loss function \cite{zhuang2022surrogate}, friendly adversary \cite{li2023enhancing}, and training efficiency \cite{du2022efficient, liu2022towards, du2022sharpness,zhao2022ss,jiangadaptive}.

% \paragraph{Efficient Sharpness-aware Minimization.}
% As SAM requires two consecutive gradient propagation for solving the min-max problem,
% its training speed is $2\times$ slower than that of regular SGD training. Many methods have been developed to improve the training efficiency \cite{du2022efficient, liu2022towards, du2022sharpness}. For example, \cite{du2022efficient} proposed ESAM that adopts two acceleration strategies for SAM's two updating steps and achieves up to 30\% computational saving. \cite{liu2022towards} proposed LookSAM, which periodically calculates the inner gradient ascent step to reduce the additional computation. 
% \cite{mi2022make} accelerates the SAM's training by introducing a sparsified binary mask for perturbations.
% \cite{du2022sharpness} proposed a novel trajectory loss to replace the gradient accent step of SAM and achieve almost ``free'' sharpness-aware minimization. 
% Different from previous approaches, we improve the training efficiency of SAM by parallelizing the two consecutive gradient steps in each iteration, allowing almost the same training speed as regular training with comparable or even better generalization.

% Different from previous approaches, we improve the training efficiency by parallelizing the two consecutive gradient computations of SAM, allowing almost the same training speed as regular training with improved generalization due to a wider flat minima.
\vspace{2mm}
\noindent
\textbf{Understanding SAM.}
Despite the empirical success of SAM across various tasks, a deep understanding of its generalization performance is still limited.
Foret et al. \cite{foret2020sharpness} explain the success of SAM based on a PAC-Bayes generalization bound. However, their analysis does not distinguish adversarial or random perturbation and whether the perturbation is computed based on some or all training samples.
Andriushchenko and Flammarion \cite{andriushchenko2022towards} investigate the implicit bias of SAM for diagonal linear networks. 
Wen et al. {\cite{wen2022sharpness}} demonstrate that SAM minimizes the top eigenvalue of Hessian in the full-batch setting.
% Thomas M{\"o}llenhoff and Mohammad Emtiyaz Khan \cite{lenhoff2023sam} connect SAM with the relaxation of the Bayes objective.
Chen et al. \cite{chen2023does} study the SAM for non-smooth convolutional ReLU networks and explain the success of SAM in its ability to prevent noise learning. While previous works primarily focus on simplified networks or ideal loss objectives, we aim to deepen the understanding of SAM by undertaking a deep investigation into the key components that contribute to its practical generalization improvement.



% \paragraph{Regularization Methods.} 
% Various regularization methods play a fundamental role in generalization improvements.
% Apart from the well-known regularization techniques such as weight decay \cite{krogh1991simple}, dropout \cite{srivastava2014dropout}, label smoothing \cite{szegedy2016rethinking} and normalization \cite{ioffe2015batch, ba2016layer}, MixUp \cite{zhang2018mixup} encourages the network to behave linearly across different samples. 
% Flooding \cite{ishida2020we} directly forces the training loss to stay above zero to avoid meaningless overfitting. 
% \cite{zhao2022penalizing} penalized the gradient norm of loss function during optimization to efficiently improve the generalization.
% Data augmentation techniques, such as Cutout \cite{devries2017improved}, CutMix \cite{yun2019cutmix}, RandAugment \cite{cubuk2020randaugment} and AutoAugment \cite{cubuk2019autoaugment}, also regularize deep networks from overfitting by diversifying the training data, thereby improving the performance.
% We impose regularization by requiring the network to perform well under random weight perturbations. Our method is orthogonal to previous regularization methods, and it is possible to combine them to attain further generalization improvements.

\section{Preliminaries}
\label{sec:preliminary}

Let $f(\boldsymbol{x};\boldsymbol{w})$ parameterized by  $\boldsymbol{w} \in \mathbb{R}^d$ be a neural network, and $L(f(\boldsymbol{x}_i;\boldsymbol{w}), \boldsymbol{y}_i)$ ($L_i(\boldsymbol{w})$ for short)   denote the loss to measure the discrepancy between the  prediction $f(\boldsymbol{x}_i;\boldsymbol{w})$ and the ground-truth label $\boldsymbol{y}_i$.  Given a dataset $\mathcal{S}={ (\boldsymbol{x}_i,\boldsymbol{y}_i) }_{i=1}^n$ i.i.d. drawn from a data distribution $\mathcal{D}$, the empirical training loss is often defined as 
\begin{equation}
   L(\boldsymbol{w})= \frac{1}{n}\sum\nolimits_{i=1}^nL_i(\boldsymbol{w}). 
\end{equation}
To solve this problem, one often uses SGD  or Adam to optimize it.  To further improve the generalization performance, 
SAM~\cite{foret2020sharpness} aims to minimize the worst-case loss within a defined neighborhood  for guiding the training process towards flat minima. The objective function of SAM is given by:
\begin{equation}
	L^{\rm SAM}(\boldsymbol{w})= \max\nolimits_{\| \boldsymbol{\epsilon} \|_2 \le \rho} L(\boldsymbol{w}+\boldsymbol{\epsilon}),
	\label{equ:sam}
\end{equation}
where $\rho$ denotes the neighborhood radius. Eqn.~\eqref{equ:sam} shows that  SAM seeks to minimize the maximum loss over the neighborhood surrounding the current weight  $\boldsymbol{w}$. By doing so, SAM encourages the optimization process to converge to flat minima which often enjoys better generalization  performance~\cite{hochreiter1997flat,dinh2017sharp, li2018visualizing,zhou2020towards}.

% To compute the worst perturbation $\boldsymbol{\epsilon}_s$, SAM approximates  Eqn.~\eqref{equ:sam} via first-order expansion as follows:
To efficiently optimize $	L^{\rm SAM}(\boldsymbol{w})$, SAM first approximates  Eqn.~\eqref{equ:sam} via first-order expansion and compute the worst-case perturbation $\boldsymbol{\epsilon}_s$ as follows:
\begin{equation}
	\boldsymbol{\epsilon}_s\approx \mathop{ \arg \max}\nolimits_{\| \boldsymbol{\epsilon} \|_2\le \rho} \boldsymbol{\epsilon}^{\top} \nabla_{\boldsymbol{w}} L(\boldsymbol{w})= \rho \frac{\nabla_ {\boldsymbol{w}} L(\boldsymbol{w})}{\| \nabla_{\boldsymbol{w}} L(\boldsymbol{w}) \|_2}.
	\label{equ:sam-first-order}
\end{equation}
% \pz{please ensure the consistency of the notations, before you use $ \nabla L_{\mathcal{B}}(\boldsymbol{w}) $ as the perturbation}
Subsequently, one can compute the gradient at the perturbed point $\boldsymbol{w}+\boldsymbol{\epsilon}_s$  as 
\begin{equation}
	\nabla L^{\rm SAM} (\boldsymbol{w}) \approx
	\nabla L (\boldsymbol{w}) |_{\boldsymbol{w}+\boldsymbol{\epsilon}_s},
\end{equation}
and follows the updating steps in SGD or Adam to update the model parameters. 
%

Before delving into our analysis, we first make some standard assumptions in stochastic optimization \cite{ghadimi2013stochastic,karimi2016linear,andriushchenko2022towards,jiangadaptive} that will be used in our theoretical analysis.
\begin{assumption}[$\beta$-smoothness]
	\label{assumption1}
	Assume the loss function $L:\mathbb{R}^d \mapsto \mathbb{R}$ to be $\beta$-smooth: there exists $\beta>0$ such that
	\begin{align}
		\| \nabla L(\boldsymbol{w})-\nabla L(\boldsymbol{v}) \|_2 \le \beta \| \boldsymbol{w}-\boldsymbol{v} \|_2, \forall \boldsymbol{w}, \boldsymbol{v} \in  \mathbb{R}^d.
	\end{align}
\end{assumption}

\begin{assumption}[Bounded variance]
	\label{assumption2}
	There exists $M>0$ for any data batch $\mathcal{B}$ such that
	\begin{align}
	\mathbb{E}\| \nabla L_\mathcal{B}(\boldsymbol{w}) - \nabla L(\boldsymbol{w})  \|^2 \le M, \forall \boldsymbol{w} \in  \mathbb{R}^d.
	\end{align}
\end{assumption}

\begin{assumption}[Bounded gradient]
	\label{assumption3}
	There exists $G>0$ for any data batch $\mathcal{B}$ such that
	\begin{align}
		\| \nabla L_\mathcal{B}(\boldsymbol{w}) \| \le G, \forall \boldsymbol{w} \in  \mathbb{R}^d.
	\end{align}
\end{assumption}



\section{Empirical Analysis of SAM}
%\subsection{Delving into the components of the accent step}
\label{sec:investigation}
Here  we conduct a set of experiments to identify the effective components in the weight perturbation that contributes to SAM's improved generalization performance. 
To this end, we decompose the perturbation direction  $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ in SAM   into two orthogonal components. The first one is the full gradient component $\mathrm{Proj}_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w}) $ which  is the projection  onto the full gradient direction, i.e., 
\begin{equation*}
\mathrm{Proj}_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w}) = \cos(\nabla L(\boldsymbol{w}), L_{\mathcal{B}}(\boldsymbol{w})) \nabla L(\boldsymbol{w}),
\end{equation*}
where $\cos(\cdot, \cdot)$ denotes the cosine function.  
Another one is  the residual projection, i.e., the stochastic gradient noise component which is defined as    
\begin{equation}\label{equ:residual-projection}
\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w}) =  \nabla L_{\mathcal{B}}(\boldsymbol{w})  - \mathrm{Proj}_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w}).
\end{equation}
In the following, we will investigate the effects of these two orthogonal components to the performance of SAM.  
%Surprisingly, we empirically observe  that removing the full gradient component via setting perturbation $\boldsymbol{\epsilon}_s = \rho \frac{\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})}{\|\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})\|}$ during each training iteration had almost no impact on generalization performance; in some cases, such full gradient component even results in a detrimental effect.


% \pz{please keep consistency, in introduction you use perturbation while here you use ``accent step ".  Always using the same one. }

\subsection{Effect of Full Gradient Component} %Useless
Here we investigate the impact of the full gradient component
% $\mathrm{Proj}_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$ 
% defined in Eqn.~\eqref{adsaerw} 
to the generalization performance of SAM. 
% To this end, we plug SAM into SGD for this investigation.
Specifically, for each training iteration, we set the perturbation $\boldsymbol{\epsilon}_s$  as $\boldsymbol{\epsilon}_s=\rho \frac{\nabla L(\boldsymbol{w})}{\|\nabla L(\boldsymbol{w}\|}$, and then follow the minimization step in vanilla SAM to minimize the perturbed training loss. For brevity, this modified SAM version is called ``SAM-full" since it uses the full gradient direction as the perturbation direction. 
Then we follow the standard training settings of SAM and compare the performance of SGD/AdamW, SAM, and SAM-full in training from scratch and transfer learning tasks. See more training details in Sec.~A5.
% \cref{sec:more_investigation_details}}.

% Then we follow the standard training settings of SAM to evaluate plain SGD, SAM, and SAM-full by using ResNet18 on CIFAR-100 datasets. \pz{See more training details in Appendix.}
 
 \cref{fig:sam-fb} summarizes the results. One can observe that SAM significantly outperforms the base optimizer in most scenarios, except for the Flower-102 dataset~\cite{nilsback2008automated}, where the training data is very limit (see  \cref{sec:transfer} for more discussion). However, SAM-full does not enhance the performance of base optimizer in most cases, and even severely impairs the performance when the training samples are small (e.g. on the  Flower-102 dataset). This implies that 1) utilizing full gradient 
% component
% $\mathrm{Proj}_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$ 
as the perturbation indeed does not improve generalization and can even have negative effects; 2) the effectiveness of SAM primarily arises from the presence of stochastic gradient noise component  $\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$ within the minibatch gradient $\nabla L_{\mathcal{B}}(\boldsymbol{w})$.  


% Figure \ref{fig:sam-fb} summarizes the classification accuracy results. One can observe that  SAM outperforms its base-optimizer SGD by a remarkable margin on all training settings which is also observed in many other works \pz{citations}. But with the same SGD as the base optimizer, SAM-full does not improve SGD in most cases, and even impairs the classification performance of SGD.  This means that 1) taking full gradient component $\mathrm{Proj}_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$ as the perturbation indeed does not improve SAM; 2) the effectiveness of SAM primarily arises from the presence of stochastic gradient noise component  $\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$ within the minibatch gradient $\nabla L_{\mathcal{B}}(\boldsymbol{w})$.  

To provide more evidence, we further modify the perturbation step in SAM by increasing the minibatch size through gradually adding more training samples. As illustrated in  \cref{fig:sam-strength}, we use a minibatch $\mathcal{B}'$ with size $k\times 128$ to compute the perturbation in SAM, where $k$ is selected from $\{1, 2, 3, \cdots, 10\}$. However, we maintain the use of a minibatch $\mathcal{B}$ of size 128 for the second minimization step ($\mathcal{B} \subseteq \mathcal{B}'$), following the standard SAM. 
% , and always follow vanilla SAM to use a minibatch of 128 for the second minimization step, i.e., $k=1$ recovers the vanialla SAM. 
% It means that 
For the perturbation $\boldsymbol{\epsilon}_s = \rho \frac{\nabla L_{\mathcal{B}'}(\boldsymbol{w})}{\|\nabla L_{\mathcal{B}'}(\boldsymbol{w})\|}$, its direction gradually aligns more closely with
% becomes more close to 
the full gradient direction along with increment of $k$. 
Consequently, as the minibatch size grows, the contribution of the full gradient component in the perturbation step becomes stronger, while the residual stochastic gradient noise component weakens. This analysis helps to reveal the perturbation effects of the full gradient direction in SAM's perturbation.
% That is, as the minibatch size grows, the full gradient component in the perturbation step is strengthen, while the residual stochastic gradient noise component is weaken. This also helps to reveal the perturbation effects of full gradient direction to SAM.
% Then we evaluate this SAM by using  \pz{XX network on XXX dataset}.

% To provide more evidence, we use vanilla SAM, but adopts larger minibatch size in the perturbation step.  As illustrated in Figure \ref{fig:sam-strength}, we use a minibatch size of $k\times 128$ to compute the pertubation in SAM, and always follow vanilla SAM to use a minibatch of 128 for the second minimization step, where $k$ is selected from $\{1, 2, 3, \cdots, 10\}$. It means that for the perturbation $\boldsymbol{\epsilon}_s = \rho \frac{\nabla L_{\mathcal{B}}(\boldsymbol{w})}{\|\nabla L_{\mathcal{B}}(\boldsymbol{w})\|}$ in vanilla SAM, its direction becomes more close to the full gradient direction along with increment of $k$. That is, as the minibatch size grows, the full gradient component in the perturbation step is strengthen, while the residual stochastic gradient noise component is weaken.  So this also helps to reveal the perturbation effects of full gradient direction to SAM. Then we evaluate this SAM by using  \pz{XX network on XXX dataset}.

By observing \cref{fig:sam-strength}, one can find that when minibatch size increases, the classification accuracy  gradually decreases. See more similar experimental results in Sec.~A5.
% \cref{sec:more_investigation_details}.  
All these results together   indicate  that  strengthening the full gradient component in the perturbation steps impairs the generalization performance of vanilla SAM. 

 
%As illustrated in Figure \ref{fig:sam-strength}, we progressively increase the batch size of the first accent step. It is important to note that the original batch data are retained throughout this process. As the batch size grows, the full gradient component in the accent step is strengthen, while the residual stochastic gradient noise component is weaken. We observe that the final performance gradually decreases, indicating that strengthening the full gradient component in the accent steps impairs generalization. 
%
%
%The rationale behind this phenomenon can be attributed to the fact that the full gradient accent component can hinder the training process by increasing the loss over the entire dataset. This, in turn, adversely affects the generalization performance, as detailed in Section \ref{sec:investigation}.    \pz{This one need to to think and revise in the final stage.}
%
%In alignment with the initial objective of SAM's min-max optimization approach, we modify the first accent step by using the full gradient (SAM-full), as illustrated in Figure \ref{fig:sam-fb}. However, our observations indicate that this modification does not yield any discernible improvement in generalization when compared to plain SGD.
%This finding implies that SAM's generalization does not rely on optimizing the sharpness of the global loss objective. Moreover, including the full gradient accent component in the accent step does not significantly enhance the generalization capabilities.
%
%To provide further evidence, we conducted an additional experiment to demonstrate that increasing the strength of the full gradient component in perturbations negatively affects generalization. 
%As illustrated in Figure \ref{fig:sam-strength}, we progressively increase the batch size of the first accent step. It is important to note that the original batch data are retained throughout this process. As the batch size grows, the full gradient component in the accent step is strengthen, while the residual stochastic gradient noise component is weaken. We observe that the final performance gradually decreases, indicating that strengthening the full gradient component in the accent steps impairs generalization. 
%% \pz{this part should be combined with the first part?}


\subsection{Effects of Stochastic Gradient Noise Component}
% \pz{In the introduction, we say the perturbation contains  stochastic gradient noise and the full gradient. So here you also should show the effects of these two terms? instead of a new term. This makes the paper consistent  }
% \pz{please follow the above writing to rewrite this section}

To delve into the role of the stochastic gradient noise component in SAM's generalization improvement, we first replace the gradient noise component of the current minibatch data with another random batch. We term this modified version ``SAM-db'' as it employs two different batches of data for SAM's two gradient steps. As illustrated in \cref{fig:sam-db},  we observe that SAM-db exhibits no significant improvement in generalization when compared to plain SGD. It is important to note that in this scenario, the full gradient component can be considered analogous to original SAM (rigorously in terms of expectation), with the sole  distinction being the replacement of stochastic gradient noise component from the current minibatch data with another random batch. This substitution ultimately impedes  generalization. Therefore, we conclude that the stochastic gradient noise originating from the \emph{current} minibatch in perturbation plays a pivotal role in determining generalization.

% To further confirm the importance of the stochastic gradient noise component in the current batch gradient, 
To further solidify this observation, 
we modify SAM by setting the perturbation $\boldsymbol{\epsilon}_s$ as $\boldsymbol{\epsilon}_s = \rho \frac{\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})}{\|\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})\|}$. In other words, we only utilize the stochastic gradient noise component for SAM's perturbation. We refer to this modified version as "SAM-noise".
% , i.e., we solely utilize the stochastic gradient noise component for SAM's perturbation. We term this modified version as ``SAM-noise''. 
As illustrated in \cref{fig:sam-db}, we observe that SAM-noise not only restores the generalization performance of SAM and but even exhibits a notable  enhancement.
This result highlights that exclusively utilizing the gradient noise component for SAM's perturbation can further enhance its generalization ability, thereby inspiring the subsequent development of our F-SAM algorithm.
% This result demonstrates that solely utilizing the gradient noise component for SAM's perturbation can further strengthen SAM's generalization, inspiring our subsequent F-SAM algorithm.

% This shows that solely utilizing the gradient noise component for SAM's perturbation can further strengthen SAM's generalization, which inspire our follow F-SAM algorithm.


% we observe that solely utilizing the gradient noise component further enhance SAM's generalization. 


% Therefore, we conclude that the stochastic gradient noise originating from the batch gradient in perturbation plays a pivotal role in determining generalization. 


% We consider two modifications to SAM: 1) SAM-noise by only keeping the stochastic gradient noise component in SAM's perturbation and 2) SAM-db by replacing with a randomly selected batch data the minibatch data for the perturbation step. 

% In \cref{fig:sam-db}, 

% In the previous subsection, we have shown that the full gradient component in the accent step contributes little to the generalization improvement, and in certain cases, it can even have a negative impact. Subsequently, we demonstrate that the residual projection, i.e., the gradient noise of the \emph{current} batch data, determines generalization. To further investigate this concept, we introduce a modification to the initial accent step in the SAM algorithm by incorporating a randomly selected batch data (SAM-db), as illustrated in \cref{fig:sam-db}. However, we do not observe any significant enhancement in generalization when compared to plain SGD. It is important to note that in this scenario, the full gradient component can be regarded as similar to original SAM (rigorously in terms of expectation), with the only distinction being the replacement of stochastic gradient noise from the current batch data with another random batch. This substitution ultimately hampers generalization. Therefore, we conclude that the stochastic gradient noise originating from the \emph{current} batch in perturbation plays a pivotal role in determining generalization.

% We then conduct an experiment by utilizing two different batches of data for the two steps in SAM, as illustrated in Figure \ref{fig:sam-db}. Still, we do not observe any notable improvement in generalization compared with plain SGD with this modification.
% This finding suggests that in addition to the full gradient accent component, the residual accent component must be precisely consistent with the second step in the view of training data. This implies that the residual accent component may play a crucial role in the success of SAM's practical optimization.

% We then conduct an experiment that using two different batches of data for SAM's two steps as illustrated in Figure \ref{fig:sam-db}. We still do not observe any generalization improvement. This suggests that aparting from the full gradient component, the residual accent component should be strictly consistent with the second step. This implies that the residual accent component may be the key component to the SAM's success.

% \vspace{2mm}

% Based on the analysis of previous experiments, our key findings can be summarized as follows: a) the stochastic gradient noise component in the accent step plays a crucial role in generalization; b) the full gradient component does not significantly contribute to generalization; and c) strengthening the full gradient component has the potential to negatively impact the overall generalization performance.

% \pz{After showing the effects of different terms in perturbation, you should give your overall conclusion here and also discuss the possible reasons. Then you can smoothly introduce your new method. Please follow the logic in the introduction part.}


\section{The F-SAM Algorithm}
In this section, we will present our proposed F-SAM algorithm. We begin by introducing the efficient estimation of the stochastic gradient noise component. We then describe the algorithmic steps of our proposed F-SAM. Finally, we formulate the loss objective of our F-SAM algorithm and highlight the distinctions from original SAM.


% In this section, we will elaborate on  our proposed F-SAM algorithm. We begin by introduce our modification to SAM that eliminates the full gradient component in the weight perturbation. 
% We then introduce the challenges encountered in practical network training and our proposed solutions. Next, the full F-SAM algorithm is presented with extension to the adaptive variants of SAM. Finally, we provide further insights into our F-SAM algorithm from a bi-level optimization perspective.\pz{please rewrite according to the following content}

% \subsection{Estimating  Stochastic Gradient Noise Component}
\subsection{Estimation of Stochastic Gradient Noise Component}
From the empirical results in Section~\ref{sec:investigation}, we know that the full gradient component $\mathrm{Proj}_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$ in the perturbation   impairs the performance of SAM, while  stochastic gradient noise component  $\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$ is essential to improve performance.  Accordingly, it is natural to remove the full gradient component and only use the  stochastic gradient noise component in SAM. 

To this end, we first reformulate the  stochastic gradient noise component in Eqn.~\eqref{equ:residual-projection} as 
\begin{equation}\label{equ:stochastic-noise}
	\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w}) \!=\!  \nabla L_{\mathcal{B}}(\boldsymbol{w})  - \sigma \nabla L(\boldsymbol{w}).
\end{equation}
where $\sigma = \cos(\nabla L(\boldsymbol{w}), \nabla L_{\mathcal{B}}(\boldsymbol{w})).$ From Eqn.~\eqref{equ:stochastic-noise}, one can observe that to compute  $	\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w})} \nabla L_{\mathcal{B}}(\boldsymbol{w})$, we need to compute the  minibatch gradient $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ and also the full gradient $\nabla L(\boldsymbol{w})$ at each training  iteration. For $\nabla L_{\mathcal{B}}(\boldsymbol{w})$, it is also computed in vanilla SAM and thus does not bring extra computation overhead. Regarding  $\nabla L(\boldsymbol{w})$, it is computed on the whole dataset, and thus is  computationally prohibitive in practice.

To address this issue, we resort to estimating $\nabla L_{\mathcal{B}}(\boldsymbol{w})$ with an exponentially moving average (EMA)  which accumulates the  historical minibatch gradients as follows:
\begin{align}
	\boldsymbol{m}_t = \lambda \boldsymbol{m}_{t-1} +  (1 - \lambda) \nabla L_{\mathcal{B}_t}(\boldsymbol{w}_t),
\end{align}
where $\lambda>0$  is a hyper-parameter.  This approach enables us to approximate the full gradient $\nabla L(\boldsymbol{w}_t)$ with minimal additional computational overhead. We also prove that $	\boldsymbol{m}_t $ is a good estimation to the full gradient  $\nabla L(\boldsymbol{w}_t)$ as shown in following Theorem~\ref{theoremestimation} with its proof in Appendix Sec.~A1.
% \cref{sec:proof_theoremestimation}.

% \begin{theorem}\label{theoremestimation}
% Assuming $\|\boldsymbol{w}_t - \boldsymbol{w}_{t+1}\| \leq \eta M$. The gradient $\nabla L (\boldsymbol w)$ is L-Lipschitz. For each t, 
% % $\nabla L_{\mathcal B} (\boldsymbol w_t)$ is a random vector with
% $\mathbb{E}[\nabla L_{\mathcal B} (\boldsymbol w_t)] = \nabla L (\boldsymbol w_t), \|\nabla L_{\mathcal B} (\boldsymbol w_t) -\mathbb{E}[\nabla L_{\mathcal B} (\boldsymbol w_t)] \|\leq \sigma_{\max}^2$. Set $\alpha_t \propto \lambda^{T-t}$ with $\sum_{i=1}^T \alpha_t = 1$ and assume $T>4/(1-\lambda)$. Then with probability $1-\delta$, the estimation error $\Phi = \|\sum_{t= 1}^T \alpha_t \nabla L_{\mathcal B} (\boldsymbol w_t) - \nabla L(\boldsymbol w_t)\|$ is bounded by 
% \begin{equation*}
%     \Phi \leq \mathcal{O} (\sigma_{\max} \sqrt{1-\lambda} \sqrt{\log(e^{-1/4}/\delta)} +ML\eta/(1-\lambda)).
% \end{equation*}
% This is optimized by setting $\lambda = 1-C\eta^{2/3}$, for which the bound is $\mathcal{O}({(\eta M \sigma_{\max}^2 (\log(e^{-1/4}/\delta))L)}^{1/3})$ as long as $T > C^\prime \eta^{-2/3}$.  

% % Please following Theorem 4.1 and Proposition 4.1. and 4.2 in  this work to show that "$	\boldsymbol{m}_t $ is a good estimation to the full gradient  $\nabla L(\boldsymbol{w}_t)$ "

% % \url{https://proceedings.mlr.press/v97/staib19a/staib19a.pdf}
% \end{theorem}

\begin{theorem}\label{theoremestimation}
Let Assumption \ref{assumption1}, \ref{assumption2}, and \ref{assumption3} hold.
Assuming $\|\boldsymbol{w}_t - \boldsymbol{w}_{t+1}\| \leq \gamma G$, where $\gamma$ is the learning rate and $T>4/(1-\lambda)$. With probability $1-\delta$, the estimation error $\Phi = \|\boldsymbol{m}_T - \nabla L(\boldsymbol w_T)\|$ is bounded by 
\begin{equation*}
    \Phi \leq \mathcal{O} (M \sqrt{1-\lambda} \sqrt{\log(e^{-1/4}/\delta)} +G\beta\gamma/(1-\lambda)).
\end{equation*}
It is optimized by setting $\lambda=1-C\gamma^{2/3}$ with error bound $\mathcal{O}({(\gamma GM \log(e^{-1/4}/\delta)\beta)}^{1/3})$ as long as $T > C^\prime \gamma^{-2/3}$.  

% Please following Theorem 4.1 and Proposition 4.1. and 4.2 in  this work to show that "$	\boldsymbol{m}_t $ is a good estimation to the full gradient  $\nabla L(\boldsymbol{w}_t)$ "

% \url{https://proceedings.mlr.press/v97/staib19a/staib19a.pdf}
\end{theorem}
Theorem~\ref{theoremestimation} shows that after a certain training iterations, 
the distance between the EMA $\boldsymbol{m}_t $ and  the full gradient $\nabla L(\boldsymbol{w}_t)$ is at the order of $\mathcal{O}(\gamma^{1/3})$ with properly chosen $\lambda$. This implies that using $	\boldsymbol{m}_t $ to estimate the full gradient  $\nabla L(\boldsymbol{w}_t)$ is a good choice considering the learning rate $\gamma$ decreases at a rate of $\mathcal{O} (1/\sqrt{T})$ as discussed in Theorem \ref{thm:convergence}.

In this way, the  stochastic gradient noise component in Eqn.~\eqref{equ:residual-projection} is approximated as  
 \begin{equation}\label{adasfwaasde}
 	\begin{split}
 	\mathrm{Proj}^\top_{\nabla L(\boldsymbol{w}_t)} \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)\approx   & 	\widetilde{\mathrm{Proj}}^\top_{\nabla L(\boldsymbol{w}_t)} \nabla L_{\mathcal{B}}(\boldsymbol{w}_t) \\
 	 = & \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)  - \sigma_t \boldsymbol{m}_t, 
 	\end{split}
 \end{equation}
 where $\sigma_t = \cos(\boldsymbol{m}_t, \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)).$  
% Since at the beginning of the training, $m_t$ is a rough estimation to full gradient, and both $m_t$ and $\nabla L_{\mathcal{B}}(\boldsymbol{w}_t)$ are high dimensional especially for the modern over-parameterized networks, the estimation of $\sigma_t$ is not very accurate. With more training, as shown in  Theorem~\ref{theoremestimation},   $m_t$ can  estimate the full gradient more accurately, yielding an accurate estimation $\sigma_t$. So to solve the inaccurate estimation issue at the beginning of training, 
For the modern over-parameterized networks, both $\boldsymbol{m}_t$ and $\nabla L_{\mathcal{B}}(\boldsymbol{w}_t)$ are high dimensional, and their inner product is expensive. In the real network  training,  the training frameworks, e.g., PyTorch, often  uses propagation to compute the gradient for each layer. It means that one need to wait until the training framework finishes the gradient computation of all layers, and then compute $\sigma_t $ which is not efficient. More worse, the computation of cosine similarity can be less stable when the dimensionality is high and there is noise existed in the approximation $\boldsymbol{m}_t$.
So to improve the training efficiency and stability,  we set $\sigma_t$ as a constant $\sigma$, and obtain  
  \begin{equation}\label{adasfwaasadade}
 	\begin{split}
\widetilde{\mathrm{Proj}}^\top_{\nabla L(\boldsymbol{w}_t)} \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)  
=   \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)  - \sigma \boldsymbol{m}_t.
 	\end{split}
 \end{equation}
 The experimental results in Section \ref{sec:experiments} show that this practical setting achieves satisfactory performance.  In theory, we also prove that this practical setting is validated as shown in the following Lemma~\ref{theorem2} with its proof in Sec.~A2.
%  \cref{sec:proof_thm2}. 
  \begin{lemma}\label{theorem2}
 	Assuming $\boldsymbol{m}_t$ is a unbiased estimator to the full gradient $\nabla L(\boldsymbol{w}_t)$. With $\sigma=1$, we have
 	\begin{align}
 		\begin{split}
 		%	&\mathbb{E} \left \langle \hat{\boldsymbol{\mathrm{d}}}_t^s, \nabla L(\boldsymbol{w}_t) \right \rangle=0, \\
 			\mathbb{E} \left \langle \widetilde{\mathrm{Proj}}^\top_{\nabla L(\boldsymbol{w}_t)} \nabla L_{\mathcal{B}}(\boldsymbol{w}_t), \nabla L(\boldsymbol{w}_t) \right \rangle=0.
 		\end{split}
 	\end{align}
 \end{lemma}
Lemma~\ref{theorem2} indicates that $\widetilde{\mathrm{Proj}}^\top_{\nabla L(\boldsymbol{w}_t)} \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)$ is orthogonal to the full gradient $\nabla L(\boldsymbol{w}_t)$ in expectation with $\sigma=1$. It means that using $\widetilde{\mathrm{Proj}}^\top_{\nabla L(\boldsymbol{w}_t)} \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)$  as the perturbation direction can remove the effects of the full gradient $\nabla L(\boldsymbol{w}_t)$. Note that Theorem~\ref{theoremestimation} guarantees that  $\boldsymbol{m}_t$ is close the full gradient $\nabla L(\boldsymbol{w}_t)$ and thus the assumption in  Lemma~\ref{theorem2} is not restrictive. 
 
 

\subsection{Algorithmic Steps of F-SAM}
After estimating the stochastic gradient noise component in Eqn.~\eqref{adasfwaasadade}, one can use it to replace the adversarial perturbation direction in vanilla SAM, and straightforwardly obtain our proposed F-SAM. 

Specifically, for the $t$-th training iteration, following the algorithmic steps in vanilla SAM, we first define the perturbation $\boldsymbol{\epsilon}$ as follows:
\begin{align}
\boldsymbol{\epsilon}_t =  \rho \cdot \frac{\widetilde{\mathrm{Proj}}^\top_{\nabla L(\boldsymbol{w}_t)} \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)}{\|\widetilde{\mathrm{Proj}}^\top_{\nabla L(\boldsymbol{w}_t)} \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)  \|},
	\label{equ:dts}
\end{align}
where $\rho$ denotes the neighborhood radius.  
% Then we follow SAM to use SGD as its base optimizer, and adopt the updating step in SGD to minimize the pertubated training loss by taking one gradient step:
Then, following the approach of SAM, we
% utilize SGD as the base optimizer and employ the SGD update step to 
minimize the perturbed training loss by taking one gradient descent step:
\begin{equation}
\boldsymbol{w}_{t+1} = \boldsymbol{w}_t - \gamma	\nabla L_{\mathcal{B}} (\boldsymbol{w}) |_{\boldsymbol{w}_t+\boldsymbol{\epsilon}_t}. 
\end{equation}
% The algorithmic steps of F-SAM is summarized in  Algorithm
% \ref{algorithm:fsam}.
For more clear, we summarize the algorithmic steps of F-SAM in  Algorithm
\ref{algorithm:fsam}.

\begin{algorithm}[t]
	% \small
	\caption{F-SAM algorithm}
	\label{algorithm:fsam}
	\KwIn{Loss function $L(\boldsymbol{w})$,  training datasets $\mathcal{S}=\{ (\boldsymbol{x}_i,\boldsymbol{y}_i) \}_{i=1}^n$, minibatch size $b$, neighborhood size $\rho$, learning rate $\gamma$, momentum factor $\lambda$, projection constant $\sigma$} 
	\KwOut{Trained weight $\boldsymbol{w}$}  
	\BlankLine
	Initialize $\boldsymbol{w}_0$, $t\gets 0$, $\boldsymbol{m}_{-1} = \boldsymbol{0}$;\\ 
	\While{not converged}{
		Sample a minibatch data $\mathcal{B}$ of size $b$ from $\mathcal{S}$; \\
		$\boldsymbol{g}_t=\nabla L_{\mathcal{B}}(\boldsymbol{w}_{t})$;\\
		$\boldsymbol{m}_{t}=\lambda \boldsymbol{m}_{t-1}+(1-\lambda)\boldsymbol{g}_t$;\\
		$\boldsymbol{\mathrm{d}}_t=\boldsymbol{g}_t-\sigma \boldsymbol{m}_{t}$; \\
		Compute adversarial weight perturbation: \\ \quad \quad $ \boldsymbol{\epsilon}_t = \rho \frac{\boldsymbol{\mathrm{d}}_t}{\|\boldsymbol{\mathrm{d}}_t\|}$; \\
		Compute the gradient approximation  $\boldsymbol{g}$:\\
		\quad \quad $\boldsymbol{g}_t' \gets \nabla L_{\mathcal{B}}(\boldsymbol{w}_{t} + \boldsymbol{\epsilon}_t)$;
		\\
		Update $\boldsymbol{w}$ using gradient descent:\\
		\quad \quad $\boldsymbol{w}_{t+1}\gets \boldsymbol{w}_{t}-\gamma \boldsymbol{g}_t'$; \\
		$t \gets t + 1$; \\
	}
	\Return $\boldsymbol{w}_t$.
\end{algorithm}


% where we use the EMA $_t$ to approximate the full gradient $\nabla L(\boldsymbol{w})$. 
% Next, we can follow the corresponding algorithmic steps in the SAM variants to update the model parameter $\boldsymbol{w}$.

%In practice, to approximate the full gradient $\nabla L(\boldsymbol{w}_{t})$ at step $t$, we can use the following approximated expression:
%\begin{align}
%	\boldsymbol{\epsilon}_t=\rho \frac{T_w^2 \left (\nabla L_\mathcal{B}(\boldsymbol{w}_{t}) - \boldsymbol{m}_{t-1} \right )}
%	{\|T_w  \left (\nabla L_\mathcal{B}(\boldsymbol{w}_{t}) - \boldsymbol{m}_{t-1} \right )\|_2}.
%	\label{equ:perturbation-sam-variant}
%\end{align}

%
%As our improvement to SAM is applied to the accent direction, we thus can readily incorporate our methods to SAM's different adaptive variants with their respective perturbation models. We first give a unified formulation for the perturbation model of SAM's variants, including ASAM \cite{kwon2021asam} and FiserSAM \cite{kim2022fisher}. Specifically, we wish to solve the following min-max objective
%\begin{align}
%	\min_{\boldsymbol{w}} \max_{\| T_w^{-1} \boldsymbol{\epsilon} \| \le \rho} L(\boldsymbol{w}+\boldsymbol{\epsilon}),
%	\label{equ:sam-variant}
%\end{align}
%where $T_w$ is a normalization operator. For ASAM, we use $T_w=\|\boldsymbol{w}\|$, while for FisherSAM, we use $T_w=1 / \sqrt{1+\eta (\nabla L_\mathcal{B}(\boldsymbol{w}))^2}$. It is worth noting that setting $T_w=1$ corresponds to the original SAM formulation. The inner maximization problem in Equation (\ref{equ:sam-variant}) can then be solved via first-order lionization as follows:
%\begin{align}
%	\boldsymbol{\epsilon}=\rho \frac{T_w^2 \nabla L_\mathcal{B}(\boldsymbol{w})}
%	{\|T_w \nabla L_\mathcal{B}(\boldsymbol{w})\|_2}.
%	\label{equ:perturbation-sam-variant}
%\end{align}
%To incorporate our improvement, we can modify Equation (\ref{equ:perturbation-sam-variant}) as follows:
%\begin{align}
%	\boldsymbol{\epsilon}=\rho \frac{T_w^2 \left (\nabla L_\mathcal{B}(\boldsymbol{w}) - \nabla L(\boldsymbol{w}) \right )}
%	{\|T_w \left (\nabla L_\mathcal{B}(\boldsymbol{w}) - \nabla L(\boldsymbol{w}) \right )\|_2},
%	\label{equ:perturbation-sam-variant}
%\end{align}
%In practice, to approximate the full gradient $\nabla L(\boldsymbol{w}_{t})$ at step $t$, we can use the following approximated expression:
%\begin{align}
%	\boldsymbol{\epsilon}_t=\rho \frac{T_w^2 \left (\nabla L_\mathcal{B}(\boldsymbol{w}_{t}) - \boldsymbol{m}_{t-1} \right )}
%	{\|T_w  \left (\nabla L_\mathcal{B}(\boldsymbol{w}_{t}) - \boldsymbol{m}_{t-1} \right )\|_2}.
%	\label{equ:perturbation-sam-variant}
%\end{align}

\subsection{A Friendly Perspective of the Loss Objective}
Here we provide an intuitive understanding on the difference between SAM and F-SAM. Given a minibatch data $\mathcal{B}$, SAM solves the inner maximization problem by seeking the following adversarial perturbation:
\begin{equation}
	\boldsymbol{\epsilon}_t^{\rm SAM}= \mathop{ \arg \max}\limits_{\| \boldsymbol{\epsilon}_t \|_2 \le \rho} L_{\mathcal{B}}(\boldsymbol{w}_t+\boldsymbol{\epsilon}_t).
\end{equation}
% \begin{align}
	%     \boldsymbol{\mathrm{d}}^{\rm SAM}=\max_{\|\boldsymbol{\mathrm{d}}\|=1} L_{\mathcal{B}_t} (\boldsymbol{w}_t+\boldsymbol{\mathrm{d}}).
	% \end{align}
On the other hand,   by observing $\widetilde{\mathrm{Proj}}^\top_{\nabla L(\boldsymbol{w}_t)} \nabla L_{\mathcal{B}}(\boldsymbol{w}_t)  $ defined in Eqn.~\eqref{adasfwaasadade}, F-SAM indeed computes the adversarial perturbation by maximizing the current minibatch loss while also minimizing the entire dataset loss:
% by maximizing the difference between the current minibatch loss and the entire dataset loss:
\begin{align*}
	{\boldsymbol{\epsilon}}_t^{\rm F \raisebox{0mm}{-}SAM}=\mathop{ \arg \max}\limits_{\| \boldsymbol{\epsilon}_t \|_2 \le \rho} L_{\mathcal{B}_t} (\boldsymbol{w}_t+\boldsymbol{\epsilon}_t)- \sigma L_{\mathcal{D}} (\boldsymbol{w}_t+\boldsymbol{\epsilon}_t).
\end{align*}
Then combining the following minimization problem, one can write F-SAM's bi-level optimization problem as
\begin{align}
\begin{split}
	\min_{\boldsymbol{w}} &~~~\mathbb{E}_{\mathcal{B}} \left [ L_{\mathcal{B}}(\boldsymbol{w}+\boldsymbol{\epsilon}_\mathcal{B})\right ] \\
	\text{s.t.}  &~~~{\boldsymbol{\epsilon}}_\mathcal{B}=\mathop{ \arg \max}\limits_{\| \boldsymbol{\epsilon} \|_2 \le \rho} L_{\mathcal{B}} (\boldsymbol{w}+\boldsymbol{\epsilon})-\sigma L_{\mathcal{D}} (\boldsymbol{w}+\boldsymbol{\epsilon}).
\end{split}
\end{align}
The insight behind is that F-SAM aims to find a adversarial perturbation that increases the loss of the current minibatch data while minimizing the impact on the loss of the other data points as much as possible, which is not optimized in the subsequent minimization step. 
% \pz{what are the benefits? why it is better?} 
% We compare the $L_{\mathcal{D}} (\boldsymbol{w}_t+\boldsymbol{\epsilon}_t)$ for SAM and F-SAM in Section X. 
One immediate benefit is that F-SAM exhibits much better robustness to larger perturbation radius as the negative impact on the loss of 
% of the perturbation to 
other data is mitigated, as discussed in Section \ref{sec:ablation}. 
% \# need a figure shows how it effects the adv loss of the current batch data and other batch data


\section{Convergence Analysis}
In this section, we analyze the convergence properties of the F-SAM algorithm under non-convex setting. 
We follow basic assumptions that are standard in convergence analysis of stochastic optimization \cite{ghadimi2013stochastic,karimi2016linear,andriushchenko2022towards}.
% with proof in Appendix Sec.~A3.
\begin{theorem}
	\label{thm:convergence}
Assume Assumption \ref{assumption1} and \ref{assumption2} hold. Let $\gamma_t=\frac{\gamma_0}{\sqrt{t}} \le {1}/{\beta}$ and the perturbation radius $\rho$ decay with square root of $t$, i.e., $\rho_t=\frac{\rho_0}{\sqrt{t}}$, we obtain:
% 	Assuming Assumption \ref{assumption1} and \ref{assumption2}, $\gamma \le 1/ \beta$, we obtain:
	\begin{align}
		\begin{split}
% 			\frac{1}{T} \sum_{t=1}^{T-1}  \mathbb{E}   \|\nabla L(\boldsymbol{w}_{t}) \|^2\le \frac{2(L(\boldsymbol{w}_0)-L(\boldsymbol{w}^*))}{\gamma T}\\+2\gamma \beta M+\rho^2\beta^2(1+\beta\gamma),
\frac{1}{{T}} \sum_{t=1}^{T}  \mathbb{E}   \|\nabla L(\boldsymbol{w}_{t}) \|^2\le
\frac{2 \left( \mathbb{E} [L(\boldsymbol{w}_{0})] - \mathbb{E} [L(\boldsymbol{w}_{T})] \right)}{\gamma_0 \sqrt{T}}\\+\frac{(2\beta M \gamma_0+ \rho_0^2 \beta^3\gamma_0+ \rho_0^2 \beta^2) \log T}{\sqrt{T}}.
		\end{split}
	\end{align}
% 	with $\boldsymbol{w}^*$ the optimal solution to $L(\boldsymbol{w})$.
\end{theorem}
\noindent
The proof can be found in Appendix Sec.~A3.
For non-convex stochastic optimization, Theorem \ref{thm:convergence} indicates that our F-SAM converges at the same rate as SAM, i.e. $\mathcal{O}(\log T/\sqrt{T})$ \cite{mi2022make,andriushchenko2022towards}, which also recovers the rates of SGD under usual condition on the step size $\gamma_t$ \cite{ghadimi2013stochastic,karimi2016linear}.
For a practical comparison of convergence between SAM and F-SAM, please refer to \cref{sec:ablation}.
% The practical convergence comparison of SAM and F-SAM can be found in \cref{sec:ablation}.
% The above theorem indicates that F-SAM can converge with ultimately the gradient norm is bounded by constants determined by the learning rate $\gamma$ as well as the perturbation radius $\rho$. This coincides with the practical scenarios.

\begin{table*}[!t]
	\centering
	\begin{tabular}{c|ccc|ccc}
		\toprule
		CIFAR-10 & SGD   &ASAM &FisherSAM &SAM &F-SAM (ours) \\
		\midrule
		\textbf{VGG16-BN} &94.96$_{\pm 0.15}$   &95.57$_{\pm 0.05}$  &95.55$_{\pm 0.08}$ &95.42$_{\pm 0.05}$ &\textbf{95.62}$_{\pm 0.04}$\\
		\textbf{ResNet-18} &96.25$_{\pm 0.06}$  &96.63$_{\pm 0.15}$ &96.72$_{\pm 0.03}$ &96.58$_{\pm 0.10}$ &\textbf{96.75}$_{\pm 0.05}$\\
		\textbf{WRN-28-10} &97.08$_{\pm 0.16}$  &97.64$_{\pm 0.13}$ &97.46$_{\pm 0.18}$ &97.32$_{\pm 0.11}$ &\textbf{97.53}$_{\pm 0.11}$  \\
		\textbf{PyramidNet-110} &97.63$_{\pm 0.09}$  &97.82$_{\pm 0.07}$ &97.64$_{\pm 0.09}$ &97.70$_{\pm 0.10}$ &\textbf{97.84}$_{\pm 0.05}$ \\
		\bottomrule
	\end{tabular}
	\caption{Test accuracy (\%) comparison of various neural networks on CIFAR-10.}
	\label{tab:cifar10}
\end{table*}


\begin{table*}[!t]
	\centering
	\begin{tabular}{c|ccc|cc}
		\toprule
		CIFAR-100 & SGD &ASAM &FisherSAM  &SAM &F-SAM (ours) \\
		\midrule
		\textbf{VGG16-BN} &75.43$_{\pm 0.19}$  &76.27$_{\pm 0.35}$ &76.90$_{\pm 0.37}$ &76.63$_{\pm 0.20}$ &\textbf{77.08}$_{\pm 0.17}$\\
		\textbf{ResNet-18} &77.90$_{\pm 0.07}$  &{81.68}$_{\pm 0.12}$ &80.99$_{\pm 0.13}$ &80.88$_{\pm 0.10}$ &\textbf{81.29}$_{\pm 0.12}$ \\
		\textbf{WRN-28-10} &81.71$_{\pm 0.13}$  &84.99$_{\pm 0.22}$ &84.91$_{\pm 0.07}$ &84.88$_{\pm 0.10}$ &\textbf{85.16}$_{\pm 0.07}$ \\
		\textbf{PyramidNet-110} &84.65$_{\pm 0.11}$  &86.47$_{\pm 0.09}$ &86.53$_{\pm 0.07}$ &86.55$_{\pm 0.08}$ &\textbf{86.70}$_{\pm 0.14}$ \\
		\bottomrule
	\end{tabular}
	\caption{Test accuracy (\%) comparison of various neural networks on CIFAR-100.}
	\label{tab:cifar100}
\end{table*}

\section{Numerical Experiments}
\label{sec:experiments}
In this section, we conduct extensive experiments over various tasks and neural network architectures to support our findings and evaluate the generalization performance of F-SAM. 
% Building on the top of base optimizers such as SGD and AdamW \cite{loshchilov2017decoupled}, we compare F-SAM with basic SAM and its two adaptive variants, ASAM and FisherSAM \cite{foret2020sharpness,kwon2021asam,kim2022fisher}. 
We first evaluate the performance of training from scratch, and then compare the performance of transfer learning setting by fine-tuning. Finally, we conduct additional studies to gain more insights into F-SAM. 



\subsection{Training From Scratch}
\textbf{~~~CIFAR.}
We first evaluate over CIFAR-10/100 datasets \cite{krizhevsky2009learning}. The network architectures we considered include VGG16-BN \cite{simonyan2014very}, ResNet-18 \cite{he2016deep}, WRN-28-10 \cite{ZagoruykoK16} and PyramidNet-110 \cite{han2017deep}. 
The first three models are trained for 200 epochs while for PyramidNet-110 we train for 300 epochs. 
We set the initial learning rate as 0.05 with a cosine learning rate schedule. The momentum and weight decay are set to 0.9 and 0.0005 for SGD, respectively. SAM, F-SAM, ASAM, and FisherSAM adopt the same setting except that the weight decay is set to 0.001 following \cite{mi2022make,li2023enhancing}.
We apply standard random horizontal flipping, cropping, normalization, and cutout augmentation \cite{devries2017improved}. For SAM, we set the perturbation radius $\rho$ as 0.1 and 0.2 for CIFAR-10 and CIFAR-100 \cite{mi2022make,li2023enhancing}. For ASAM, we adopt the recommend $\rho$ as 2 and 4 for CIFAR-10 and CIFAR-100 \cite{kwon2021asam}. For FisherSAM, we adopt the recommended $\rho=0.1$. For F-SAM, we use the same $\rho$ as SAM, and tune $\lambda=\{ 0.6, 0.9, 0.95 \}$ although all parameters outperforms SAM. We find that $\lambda=0.9$ works best for WRN-28-10 and PyramidNet-110, while $\lambda=0.6$ achieves the best for others. We simply set $\sigma=1$ for all the following experiments. Experiments are repeated over 3 independent trials.

\begin{table}[htbp]
    \centering
    \small
    \begin{tabular}{c|cc}
    \toprule
         CIFAR-10 &ASAM &F-ASAM (ours) \\
         \midrule
         \textbf{ResNet-18} &96.63$_{\pm 0.15}$ &\textbf{96.77}$_{\pm 0.11}$\\
         \textbf{WRN-28-10} &97.64$_{\pm 0.13}$ &\textbf{97.73}$_{\pm 0.04}$\\
        %  \toprule
        \midrule
         CIFAR-100 &ASAM &F-ASAM  (ours)  \\
         \midrule
         \textbf{ResNet-18} &81.68$_{\pm 0.12}$ &\textbf{81.82}$_{\pm 0.14}$ \\
         \textbf{WRN-28-10} &84.99$_{\pm 0.22}$ &\textbf{85.24}$_{\pm 0.16}$\\
    \bottomrule
    \end{tabular}
    \caption{Results on integration with ASAM.}
    \label{tab:adaptive}
\end{table}


In \cref{tab:cifar10} and \ref{tab:cifar100}, we observe that F-SAM achieves 0.1 to 0.2 accuracy improvement on CIFAR-10 and 0.2 to 0.4 improvement on CIFAR-100 in all tested scenarios. Moreover, F-SAM outperforms SAM's two adaptive variants in most cases, and in \cref{tab:adaptive}, we integrate our friendly approach to ASAM and again observe bringing consistent improvement.

\textbf{ImageNet.}
Next, we investigate the performance of F-SAM on larger scale datasets by training ResNet-50 \cite{he2016deep} on ImageNet \cite{deng2009imagenet} from scratch. We set the training epochs to 90 with batch size 128, weight decay 0.0001, and momentum 0.9. We set the initial learning rate as 0.05 with a cosine schedule \cite{li2023enhancing}. We apply basic data preprocessing and augmentation \cite{paszke2017automatic}. 
We set $\rho=0.075$ for all three SAM and variants and $\lambda=0.95$ for F-SAM.
In \cref{tab:imagenet}, we observe that F-SAM outperforms SAM and ASAM and offers an accuracy gain of 0.19 over SAM. This validates the effectiveness of F-SAM on large-scale problems.

\begin{table}[htbp]
	\centering
	\small
	\setlength{\tabcolsep}{3.5pt}
% 	\scalebox{1} {
	\begin{tabular}{c|cccc}
		\toprule
		ImageNet &SGD &ASAM &SAM  &F-SAM \\
		\midrule
		ResNet-50 &76.62$_{\pm 0.12}$ &77.10$_{\pm 0.14}$ &77.14$_{\pm 0.16}$  &\textbf{77.33}$_{\pm 0.12}$\\
		\bottomrule
	\end{tabular}
% 	}
	\caption{Test accuracy (\%) comparison on ImageNet.}
	\label{tab:imagenet}
\end{table}


\subsection{Transfer Learning}
\label{sec:transfer}
One of the fascinating training pipelines for modern DNNs is transfer learning, i.e., first training a model on a large datasets and then easily and quickly adapting to novel target datasets by fine-tuning. In this subsection, we evaluate the performance of transfer learning for F-SAM. We use a Deit-small model \cite{deit} pre-trained on ImageNet (with public available checkpoints\footnote{\url{https://github.com/facebookresearch/deit}}). We use AdamW \cite{loshchilov2017decoupled} as base optimizer and train the model for 10 epochs with batch size $128$, weight decay $10^{-5}$ and initial learning rate of $10^{-4}$. 
We adopt $\rho=0.05$ for SAM and F-SAM.
The results are shown in \cref{tab:finetuning}. We observe that F-SAM consistently outperforms SAM and AdamW by an accuracy gain of 0.1 to 0.7. 
An intriguing observation is that on small Flowers102 dataset \cite{nilsback2008automated} (with 1020 images), AdamW even outperforms SAM. 
We attribute this to the fact that when the dataset is small, the full gradient component within the minibatch gradient is more prominent, and its detrimental  impact on convergence and generalization becomes more evident.

% We attribute this to that as the dataset is small, the full gradient component in the batch gradient is significant, which prevents the convergence and potentially harms the generalization.




% \begin{table}[htbp]
%     \centering
%     \small
%     \begin{tabular}{cc|cccc}
%     \toprule
%          Datasets &Size &AdamW &SAM   &F-SAM (ours) \\
%          \midrule
%          \textbf{CIFAR-10} &50,000 &98.10$_{\pm 0.10}$ &98.32$_{\pm 0.05}$ &\textbf{98.39}$_{\pm 0.07}$\\
%         %  \hline
%          \textbf{CIFAR-100} &50,000 &88.44$_{\pm 0.10}$ &89.10$_{\pm 0.11}$ &\textbf{89.23}$_{\pm 0.12}$\\
%          \textbf{STL10} &60,000 &98.03$_{\pm 0.16}$ &98.19$_{\pm 0.06}$ &$\textbf{98.29}_{\pm 0.05}$\\
%         %  \textbf{Food101} &101,000 &85.86$_{\pm 0.09}$ &\textbf{86.65}$_{\pm 0.08}$ &\textbf{86.65}$_{\pm 0.07}$\\
%          \textbf{Flowers102} &1020 &74.82$_{\pm 0.86}$ &74.38$_{\pm 1.04}$  &$\textbf{75.15}_{\pm 0.95}$ \\
%     \textbf{OxfordIIITPet}  &3680 &92.42$_{\pm 0.43}$ &92.70$_{\pm 0.26}$ &\textbf{92.83}$_{\pm 0.11}$ \\
%     \bottomrule 
%     \end{tabular}
%     \caption{Test accuracy (\%) comparison of various neural networks on CIFAR-10.}
%     \label{tab:finetuning}
% \end{table}

\begin{table}[htbp]
    \centering
    \small
    \begin{tabular}{c|cccc}
    \toprule
         Datasets  &AdamW &SAM   &F-SAM (ours) \\
         \midrule
         \textbf{CIFAR-10}  &98.10$_{\pm 0.10}$ &98.30$_{\pm 0.05}$ &\textbf{98.39}$_{\pm 0.07}$\\
        %  \hline
         \textbf{CIFAR-100}  &88.44$_{\pm 0.10}$ &89.10$_{\pm 0.11}$ &\textbf{89.23}$_{\pm 0.12}$\\
        %  \textbf{STL10}  &98.03$_{\pm 0.16}$ &98.19$_{\pm 0.06}$ &$\textbf{98.29}_{\pm 0.05}$\\
        %  \textbf{Food101} &101,000 &85.86$_{\pm 0.09}$ &\textbf{86.65}$_{\pm 0.08}$ &\textbf{86.65}$_{\pm 0.07}$\\
    \textbf{Standford Cars}  &74.78$_{\pm 0.09}$ &75.39$_{\pm 0.05}$ &\textbf{75.76}$_{\pm 0.14}$ \\
         \textbf{Flowers102}  &74.82$_{\pm 0.36}$ &74.38$_{\pm 0.24}$  &$\textbf{75.15}_{\pm 0.35}$ \\
    % \textbf{OxfordIIITPet}  &92.42$_{\pm 0.43}$ &92.70$_{\pm 0.26}$ &\textbf{92.83}$_{\pm 0.11}$ \\
    \bottomrule 
    \end{tabular}
    \caption{Results on transfer learning by fine-tuning.}
    \label{tab:finetuning}
\end{table}

\subsection{Additional Studies}
\label{sec:ablation}

\subsubsection{Robustness to label noise}
\begin{table}[htbp]
	\setlength{\tabcolsep}{3.5pt}
    \centering
    \small
    \begin{tabular}{c|cccc}
    \toprule
        {Rates} &\textbf{20\%}  &\textbf{60\%} &\textbf{70\%} &\textbf{80\%}\\
    \midrule
    SGD & &52.21$_{\pm 0.23}$ &39.31$_{\pm 0.13}$ &27.86$_{\pm 0.53}$\\
    SAM &95.27$_{\pm 0.09}$ &90.08$_{\pm 0.09}$  &84.89$_{\pm 0.10}$ &31.73$_{\pm 3.37}$ \\
    F-SAM &\textbf{95.42}$_{\pm 0.08}$ &\textbf{90.47}$_{\pm 0.05}$ &\textbf{86.48}$_{\pm 0.07}$ &\textbf{59.39}$_{\pm 1.77}$ \\
    \bottomrule
    \end{tabular}
    \caption{Results under label noise on CIFAR-10 with ResNet-18.}
    \label{tab:my_label}
\end{table}

\subsubsection{Robustness to perturbation radius}
One deficiency for SAM is its sensitive to the perturbation radius, which may require choosing different radii for optimal performance on different datasets. Especially, an excessively large perturbation radius can result in a sharp decrease in generalization performance. We attribute a portion of this over-sensitivity to the impact of the adversarial perturbation derived from the current minibatch data on the other data samples. Such an impact can be more obvious when the perturbation radius increases as the magnitude of the full gradient component grows correspondingly. 
In our F-SAM, such impact on other data samples is eliminated as much as possible, and thus, we can expect that it is more robust to the choices of the perturbation radius. In \cref{fig:different-rho}, we plot the performance of SAM and F-SAM under different perturbation radii. We can observe that F-SAM is much less sensitive to $\rho$ than SAM. Especially on larger perturbation radius, the performance gain of F-SAM over SAM is more significant.
For example, when $\rho$ is set to 2x larger than the optimal on CIFAR100, SAM's performance suffers a sharp drop from $80.88\pm0.10$ to $78.83\pm 0.12$, but F-SAM still achieves a good performance of $80.30\pm 0.10$. This confirms F-SAM's improved robustness to perturbation radius.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.45\linewidth}
 \centering
  \includegraphics[width=1\linewidth]{figure/sam-large-radius-c10.pdf}
 \end{subfigure}
    \hspace{0.03in}
    \begin{subfigure}{0.45\linewidth}
 \centering
  \includegraphics[width=1\linewidth]{figure/sam-large-radius-c100.pdf}
    % \caption{ResNet-18 on CIFAR-100.}  
    % \label{fig:sam-db}
 \end{subfigure}
 \vspace{-2mm}
    \caption{Results under different perturbation radii $\rho$. 
    % F-SAM is less sensitive to $\rho$ compared with SAM especially on larger $\rho$. 
    }
    \label{fig:different-rho}
\end{figure}

\vspace{-4mm}

\subsubsection{Results on different batch sizes}
As the main claim of this paper is that the full gradient component existing in SAM's adversarial perturbation does not contribute to generalization and may have detrimental effects.
As the training batch size increases, the corresponding full gradient component existing in the minibatch gradient can be strengthened. Thus, the improvement of F-SAM from removing the full gradient component could be more obvious. 
In \cref{fig:largebz}, we compare the performance of SGD, SAM, and our F-SAM under batch sizes from $\{ 128, 512, 2048 \}$ while keeping other hyper-parameters unchanged. 
We observe that the performance gain of F-SAM over SAM increases significantly as the batch size increases. This further validates our findings and supports the effectiveness of removing the full gradient component.

\noindent
\textbf{Connection to m-sharpness.} 
We would like to relate our removing the full gradient component to the intriguing $m$-sharpness in SAM, which is defined as the search for an adversarial perturbation that maximizes the sum of losses over sub-batches of $m$ training points \cite{foret2020sharpness}. This phenomenon emphasizes the importance of using a small $m$ to effectively improve generalization \cite{foret2020sharpness,andriushchenko2022towards, behdin2022improved}.
It is worth noting that by utilizing a small sub-batch, one implicitly suppresses the effects of the full gradient component. Hence, our findings can provide new insights into understanding $m$-sharpness.
% which we leave for future works to explore further.

\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{figure/sam-large-bz.pdf}
    \vspace{-3mm}
    \caption{Performance comparison with different batch sizes.}
    \label{fig:largebz}
\end{figure}

\subsubsection{Training curves}
\label{sec:pratical_training_curves}
In \cref{fig:training_curves}, we compare the training curves of SAM and F-SAM. We observe that F-SAM achieves a faster convergence than SAM especially on the initial stage. This is because at the initial stage, the proportion of the full gradient component in the minibatch gradient is more significant,and hence removing this component to facilitate convergence in F-SAM has a more pronounced effect. Moreover, as the perturbation radius grows (2x in this case), the magnitude of the full gradient component in $\boldsymbol{\epsilon}_s$ also grows. 
This can significantly hinder the convergence of SAM and degrade its performance. In contrast, F-SAM is able to mitigate this undesired effects and maintain a good performance.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.45\linewidth}
 \centering
  \includegraphics[width=1\linewidth]{figure/trainingloss.pdf}
 \end{subfigure}
    \hspace{0.03in}
    \begin{subfigure}{0.45\linewidth}
 \centering
  \includegraphics[width=1\linewidth]{figure/testacc.pdf}
 \end{subfigure}
 \vspace{-2mm}
    \caption{Training curves on CIFAR-100 with ResNet-18. }
    \label{fig:training_curves}
\end{figure}

% \subsubsection{Loss surfaces and Hessian spectrum}

% \begin{table*}[]
	%     \centering
	%     \begin{tabular}{c|cccc}
		%     \toprule
		%          CIFAR-10 & SGD &SAM   &F-SAM (ours) \\
		%          \midrule
		%          \textbf{VGG16-BN} &94.96$_{\pm 0.15}$ &95.42$_{\pm 0.05}$   &\textbf{95.62}$_{\pm 0.04}$\\
		%          \textbf{ResNet-18} &96.25$_{\pm 0.06}$ &96.58$_{\pm 0.10}$ &\textbf{96.74}$_{\pm 0.05}$\\
		%          \textbf{WRN-28-10} &97.08$_{\pm 0.16}$ &97.32$_{\pm 0.11}$  &\textbf{97.53}$_{\pm 0.11}$  \\
		%          \textbf{PyramidNet-110} & &97.82$_{\pm 0.10}$ &\textbf{97.96}$_{\pm 0.08}$ \\
		%     \bottomrule
		%     \end{tabular}
	%     \caption{Test accuracy (\%) comparison of various neural networks on CIFAR-10.}
	%     \label{tab:my_label}
	% \end{table*}



% \begin{table}[]
	%     \centering
	%     \begin{tabular}{cccc}
		%     \toprule
		%          Datasets & &ASAM &F-ASAM  \\
		%          \midrule
		%          CIFAR-10 &\textbf{ResNet-18}   &96.63$_{\pm 0.15}$ \\ &\textbf{WRN-28-10} &\textbf{96.73}$_{\pm 0.11}$\\
		%          \midrule
		%          \textbf{ResNet-18} &\\
		%          \textbf{WRN-28-10} & \\
		%     \bottomrule
		%     \end{tabular}
	%     \caption{Combining with different SAM-variants on CIFAR-10.}
	%     \label{tab:my_label}
	% \end{table}

% \begin{table}[]
% 	\centering
% 	\begin{tabular}{c|cc}
% 		\toprule
% 		CIFAR-10 &\textbf{ResNet-18} &\textbf{WRN-28-10} \\
% 		\midrule
% 		ASAM   &96.63$_{\pm 0.15}$ &97.64$_{\pm 0.13}$\\
% 		F-ASAM &\textbf{96.73}$_{\pm 0.11}$ &\textbf{97.73}$_{\pm 0.04}$\\
% 		\midrule
% 		FisherSAM &96.68$_{\pm 0.12}$ &97.60$_{\pm 0.06}$\\
% 		F-FisherSAM&\textbf{96.77}$_{\pm 0.14}$ \\
% 		\bottomrule
% 	\end{tabular}
% 	\caption{Combining with different SAM-variants on CIFAR-10.}
% 	\label{tab:my_label}
% \end{table}

% \begin{table}[]
% 	\centering
% 	\begin{tabular}{c|c}
% 		\toprule
% 		CIFAR-100 & Accuracy (\%) \\
% 		\midrule
% 		ASAM &81.70$_{\pm 0.12}$\\
% 		F-ASAM &\textbf{81.82}$_{\pm 0.14}$\\
% 		\midrule
% 		FisherSAM &80.95$_{\pm 0.19}$\\
% 		F-FisherSAM &\textbf{81.17}$_{\pm 0.10}$ \\
% 		\bottomrule
% 	\end{tabular}
% 	\caption{Combining with different SAM-variants on CIFAR-100.}
% 	\label{tab:my_label}
% \end{table}






\section{Conclusion}
In this paper, we conduct an in-depth  investigation into the core components of SAM's perturbation step aiming for gaining a deeper understanding of its practical generalization improvement. By decomposing the minibatch gradient into two orthogonal components, we discover that the full gradient component in perturbation contributes minimally to generalization and may even have detrimental effects, while the stochastic gradient noise component plays a crucial role in enhancing generalization. Motivated by our findings, we propose a new variant of SAM called F-SAM to eliminate the undesirable effects of the full gradient component. Extensive experiments across various tasks demonstrate that F-SAM significantly improves the generalization performance of SAM. Our work not only provides new insights into understanding the practical success of SAM and the concept of m-sharpness but also offers inspiration for the design of more effective optimization algorithms.



==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
